Learning to Recover from Plan Execution Errors during Robot Manipulation: A Neuro-symbolic Approach

Automatically detecting and recovering from failures is an important but challenging problem for autonomous robots. Most of the recent work on learning to plan from demonstrations lacks the ability to detect and recover from errors in the absence of an explicit state representation and/or a (sub-) goal check function. We propose an approach (blending learning with symbolic search) for automated error discovery and recovery, without needing annotated data of failures. Central to our approach is a neuro-symbolic state representation, in the form of dense scene graph, structured based on the objects present within the environment. This enables efficient learning of the transition function and a discriminator that not only identifies failures but also localizes them facilitating fast re-planning via computation of heuristic distance function. We also present an anytime version of our algorithm, where instead of recovering to the last correct state, we search for a sub-goal in the original plan minimizing the total distance to the goal given a re-planning budget. Experiments on a physics simulator with a variety of simulated failures show the effectiveness of our approach compared to existing baselines, both in terms of efficiency as well as accuracy of our recovery mechanism.

==> sections/abstract.tex <==
\begin{abstract}
Automatically detecting and recovering from failures is an important but challenging problem for an autonomous robot due to the presence of perceptual noise and uncertainty in discovering the goal state. Unlike existing methods that rely on annotated failure data, our approach handles this task through self-supervised learning by exploiting the fact that actions generate localized effects around the object to which they are applied. Central to our approach is a neuro-symbolic state representation, specifically a dense scene graph, which is structured based on the objects present within the environment. This enables efficient learning of the transition function and a discriminator that not only identifies failures but also localizes them and calculates heuristic state distances.  Our technique is simple: we use the learnt transition and discriminator functions to (a) determine if a failure has occurred at any particular execution step, (b) localize the error by identifying the erroneous objects, and (c) perform a quasi-symbolic forward search over the space of scene graphs guided by the learnt heuristics to find an efficient recovery plan to the nearest state in the original plan. Experiments on a physics simulator with simulated failures during plan execution show the effectiveness of our approach compared to existing baselines.
\textbf{}

\iffalse
The ability to automatically detect and recover from failures is an important but challenging problem for an autonomous robot due to the presence of perceptual noise and uncertainty in discovering the goal state.
%
While existing approaches deal with this problem by training over data specifically annotated for failures, our goal in this work is to achieve this task, in a self-supervised manner, without requiring any such explicit annotation. 
%
Central to our approach is a neuro-symbolic object-centric representation of the state in the form of a dense scene graph. The core learning component of our approach consists of (a) neural module representing the transition function trained using data generated from an existing neuro-symbolic planner and (b) neural discriminators, trained in self-supervised manner, which not only detect failures, but also provide useful information about which objects in the scene need to be acted upon, localising the error and aiding an efficient discrepancy-aware synthesis of a recovery plan.  
%
Our technique is simple: (a) At any given execution step, we use a combination of our learned transition function and discriminator to estimate if a failure has occurred and also determine objects that need to be moved to recover from the failure (b) a recovery mechanism searches for an efficient plan to one of the states lying on the original plan %the state where failure had occurred 
using a forward search guided with learned heuristics.  
%
When the last correct state may not be the closest to the failure state, we devise an anytime version of our algorithm to search for the optimal point on the original plan to the goal.
%
Experiments on a simulated data set with a variety of failures during plan execution shows the effectiveness of our approach compared to existing baselines.
\fi
\end{abstract}

==> sections/ack.tex <==
\section{Acknowledgements}
%We thank IIT Delhi HPC facility\footnote{\emph{http://supercomputing.iitd.ac.in}} for computational resources. 
We thank anonymous reviewers for their insightful comments that helped in further improving our paper.
Parag Singla was supported by the DARPA Explainable AI (XAI) Program,
%with number \#N66001-17-2-4032, 
IBM AI Horizon Networks (AIHN) grant and
%the Visvesvaraya Young Faculty Fellowships by Govt. of India and 
IBM SUR awards.
Rohan Paul acknowledges Pankaj Gupta Young Faculty Fellowship for support. 
%This work was partially supported by the CSE Research Acceleration fund of IIT Delhi. 
We acknowledge the support of CSE Research Acceleration fund of IIT Delhi. Any opinions, findings, conclusions or recommendations
expressed in this paper are those of the authors and do
not necessarily reflect the views or official policies, either expressed or implied, of the funding agencies.


==> sections/experiment.tex <==
%%%%%%%%%%%%%%%%%%%%%% EXPERIMENTS %%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation Setup}\label{sec:experiments}

\textbf{Evaluation Corpus.} A simulated Franka Emika Panda robot~\cite{haddadin2022franka} in the PyBullet physics simulator is used to collect data set for evaluation. Scenes are synthesized by simulating $3-5$ blocks in the Physics engine by randomly sampling sizes, types and metric locations. The neural state transition model and the scene-graph discriminator are trained from $~3000$ atomic state transitions extracted from goal-reaching demonstrations (Table \ref{tab:dset-desc}).  
%
A data set of $2000+$ erroneous plan executions is created. The following errors are simulated: (i) grasping failures (e.g., object slipping from the gripper during picking or movement), (ii) erroneous action outcome (e.g., inexact placement of an object on top of another leading to instability and falling of a tower), (iii) motion planning errors (e.g., unexpected collision between the arm and partially constructed assembly due to uncertainty in exact object locations), (iv) actions of an external agent (e.g., a human unexpectedly moves blocks randomly or aids plan progress by pro-actively performing the next action) and (v) explicit errors (e.g., random application of disturbance forces or swapping of objects). Resulting plans possess $1-10$ steps, the scenes have $5-10$ objects with upto $5$ errors at a single step. 

\begin{table}[ht]
    \centering
    \caption{Evaluation dataset characteristics.}
    \begin{tabular}{|l|c|c|c|c|}
    \hline
     Index & Size & Error Types & \#Objects & Plan len \\
    \hline
    Data set I & 750+ & (1-5) on random step & 5 & 5 \\
    \hline
    Data set II & 1300+ & 1 on each step & 5 & 1-8 \\
    \hline
    Data set III & 200+ & 5 on random step & (6-10) & 5 \\
    \hline
    \end{tabular}
    \label{tab:dset-desc}
\end{table}

\textbf{Baselines and Ablations. }\label{subsec:baseline}
The proposed approach (named Ours (without anytime algorithm)) is compared with two baseline approaches: (i) \emph{RePlan:} a neuro-symbolic planner inspired by PDSketch \cite{mao2022pdsketch} that performs a symbolic heuristic search as its planning framework. This planner uses a learned transition function and a goal-check function. Even though it can detect whether or not it has reached the goal state, it lacks the reasoning to detect whether an error has occurred at some intermediate state or not. For a fair comparison, the baseline is augmented with the discrepancy predictor (in the form of our $=_\mathcal{S}$) and a domain-specific heuristic ($\mathcal{D}$). (ii) \emph{NoFree:} our planner except the \textit{free}-space transformer network. Even though this planner is \textit{discrepancy}-aware, the action space is large and cannot be effectively pruned in general settings as it lacks the ability to reason over the metric space (for block un-stacking etc.), which otherwise was not needed due to the \textit{free}-space transformer inspired from~\cite{liu2022structdiffusion}. For a fair comparison, the action pre-conditions and object association between different states are known. At last, we also compare Ours with the anytime variant of the algorithm (named Ours ($\backslash$w Anytime)) to compare the efficiency of plan length. 

We also evaluated an RL-based reactive planner ~\cite{li2020towards}, trained using \emph{Soft Actor Critic (SAC)} with replay buffer. The learned goal-conditioned policies performed poorly (after $12$ hours of training) in terms of goal-reaching rate, attributed largely to the domain complexity. The planner had a 6\% success rate in predicting single-step plans for scenes containing three objects, as compared to 3.7\% by a random planner.

%%%% Metrics for evaluating error recovery
\textbf{Evaluation Metrics. } We adopt the following metrics: (i) \textit{Detection Accuracy}: Detecting if the current state after an action execution is erroneous  (ii) \textit{Recovery Accuracy $(Rec.\%)$}: Given correct detection, generating a correct recovery plan which on execution leads to the intended intermediate state (iii) \textit{Length of recovery plan ($L$)}: To evaluate if the returned plan is efficient. It is measured relative to the number of introduced errors in the current state $(L/N_{err})$ and the length of the most optimal recovery plan possible $(L/L_{opt})$. (iv) \textit{Time to generate recovery plan ($T$)}: To evaluate if the recovery planning is fast. It is measured relative to the number of introduced errors in the current state $(T/N_{err})$ and the length of the most optimal recovery plan possible $(T/L_{opt})$. (v) \textit{Fraction of plan completed $(Compl.\%)$}: Evaluating the fraction up to which the original plan could be completed by successfully recovering from errors.

% New Experimental Setup section
% \section{Experimental Setup}\label{sec:experiments}

% \textbf{Training and Evaluation Corpora. } 
% %
% A corpus is collected in a PyBullet tabletop environment using a simulated Franka Emika Panda robot arm~\cite{haddadin2022franka}. The training data set for neural predictor and discriminator consists of a corpus of 3000+3000+ initial and final world states along with a single-step natural language instruction. 
% %
% Scenes are generated for a tabletop workspace with 3−53-5 blocks of varying colors and shapes and placed at randomized world locations. 
% %
% To evaluate error-recovery, a data set of 2000+2000+ robot executions with errors is generated. The following types of errors are introduced during the plan execution (i) random application of force on an object (ii) external agent intervention that interchanges the location of any two objects. The instructions consist of 1−101-10 step actions, the scenes have 5−105-10 objects 
% with a maximum of 55 errors introduced at a single step.

% \textbf{Baselines and Ablations. }\label{subsec:baseline}
% The proposed approach is compared with two baseline approaches: (i) \emph{RePlan:} a neuro-symbolic planner inspired from \cite{mao2022pdsketch} that uses A∗^*-search as its planning framework. This planner uses a transition function and the goal-check function. Even though it can detect whether or not it has reached the goal-state, it lacks the reasoning to detect whether an error has occurred at some intermediate state or not. For a fair comparison the baseline is augmented with the discrepancy predictor (in the form of our (=Z=_\mathcal{Z}) and a domain-specific heuristic (D\mathcal{D}). (ii) \emph{NoFree:} our planner except the \textit{free}-space transformer network. Even though this planner is \textit{discrepancy}-aware, the action space is large and cannot be effectively pruned in general settings as it lacks the ability to reason over the metric-space (for block un-stacking etc.) which otherwise was not needed due to the \textit{free}-space transformer inspired from~\cite{liu2022structdiffusion}. For a fair comparison, the action pre-conditions and object association between different states is known. 

% %%%% Metrics for evaluating error recovery
% \textbf{Evaluation Metrics. } We adopt the following metrics: (i) \textit{Detection Accuracy}: Detecting if the current state after an action execution is erroneous  (ii) \textit{Recovery Accuracy}: Given correct detection, generating a correct recovery plan which on execution leads to the intended intermediate state (iii) \textit{Length of recovery plan (LplanL_{plan})}: To evaluate if the returned plan is efficient. It is measured relative to the length of the most optimal recovery plan possible (Lplan/Lopt).(iv)Timetogeneraterecoveryplan(Tplan):Toevaluateiftherecoveryplanningisfast.Itismeasuredrelativetothelengthofthemostoptimalrecoveryplanpossible.(iv)Time to generate recovery plan (TplanT_{plan}):Toevaluateiftherecoveryplanningisfast.Itismeasuredrelativetothelengthofthemostoptimalrecoveryplanpossible(Tplan/Lopt)(L_{plan}/L_{opt}).(iv)Time to generate recovery plan (Tplan):Toevaluateiftherecoveryplanningisfast.Itismeasuredrelativetothelengthofthemostoptimalrecoveryplanpossible. (iv) \textit{Time to generate recovery plan (TplanT_{plan})}: To evaluate if the recovery planning is fast. It is measured relative to the length of the most optimal recovery plan possible (T_{plan}/L_{opt}). (v) \textit{Fraction of plan completed}: Evaluating the fraction up to which the original plan could be completed by successfully recovering from errors.

%%%%%%%%%%%%%%%%%%%%%% RESULTS %%%%%%%%%%%%%%%%%%%%%% 
\section{Results}\label{sec:results}
Our experiments evaluate (i) the effectiveness of the model in error recovery in relation to alternative approaches, (ii) an analysis of model components, (iii) its effectiveness in relation to an increase in plan length and compounding of errors, and recovering from multiple errors, 
%(iv) anytime version of the model, 
and (iv) qualitative results on a simulated Franka Emika Robot. 

\begin{figure*}[t]
    \centering

    \begin{subfigure}{\hsize}
    \centering
    \includegraphics[width=\textwidth, height = 2.8cm]{figures/tower_recovery_iros_qual.png}
    \caption{\footnotesize{The robot follows a 4-step plan, during which a collision leads to the falling of the formed block tower. A 3-step recovery plan follows.}}
    \label{fig:qual-1}
    
    \end{subfigure}

    \begin{subfigure}{\hsize}
    \centering
    \includegraphics[width=\textwidth]{figures/Plan_1_step_recovery_qual_iros.png}
    \caption{\footnotesize{Error in robot gripper during object movement, followed by an external agent rearranging two objects, leads to an erroneous state. The 4-step recovery includes moving an object to a collision-free space}}
    \label{fig:qual-2}
    
    \end{subfigure}
    \begin{subfigure}{\hsize}
    \centering
    \includegraphics[width=0.85\textwidth, height = 3cm]{figures/anytime_qualitative_iros.png}
    \caption{\footnotesize{Anytime recovery: An external cooperative agent helps the robot during a 4-step plan by performing two intermediate steps. The robot simply performs the last step of the plan.}}
    \label{fig:qual-2}
    \end{subfigure}

    \caption{\footnotesize{\textbf{Demonstration with a Franka Emika Robot in PyBullet Physics engine.} Detection of errors during plan execution, generation of recovery plans ultimately attaining the intended goal. Errors include (a) unexpected collisions between objects and the robot, (b) grasping failure and dropping of the block during arm movement and (c) unanticipated actions by a (cooperative) human aiding one step in plan progress. 
    Abbreviations: Y=Yellow, R=Red, G=Green, B=Blue, C=Cyan, W=White, M=Magenta, D=Dice, C=Cube, L=Lego}}
    \vspace{-0.15in}
\end{figure*}

\textbf{Plan Recovery with Single-step Errors.} 
We consider the setting where recovery is needed once during the whole execution as a result of multiple errors introduced together. Table \ref{tab:dset1} reports the performance of various models on Data set 1, where 1 to 5 errors are applied at a randomly chosen step. Note that recovery accuracy is reported for cases where error detection is correct, and other metrics involving $L_{plan}$ and $T_{plan}$ are reported when the recovery plan is correct for all the models. Figure \ref{fig:graphs} evaluates the recovery accuracy and planning time against an increasing number of errors. Note that the length of the optimal recovery plan measures the effect of introduced errors. Our model generates a recovery plan significantly quicker compared to the other two models, due to its discrepancy-awareness and effective action pruning from the free-space network. A low recovery time leads to a high recovery accuracy, due to the availability of an overall planning time budget ($\sim30s$). 

\begin{table}[!t]
    \centering
    \caption{Performance comparison with multiple errors introduced at a single step.}
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
         Model & Recovery \% &  $L/N_{err}$ & $L/L_{opt}$ & $T/N_{err}$ & $T/L_{opt}$  \\ 
         %Model & Recovery \% &  Plan per Error & Lplan/LoptL_{plan}/L_{opt} & Tplan/NerrT_{plan}/N_{err} & Tplan/LoptT_{plan}/L_{opt}  \\ 
         \hline
         \hline
         Ours & \textbf{99.61} & 1.48 & 1.06 & \textbf{0.06s} & \textbf{0.04s} \\ 
         \hline 
         RePlan & 98.83 & 1.48 & 1.07 & 0.18s & 0.11s \\
        \hline 
         NoFree & 87.83 & 1.46 & 1.05 & 0.75s & 0.42s \\ 
        %  Ours & \textbf{99.61} & 1.53 & 1.13 & \textbf{0.10s} & \textbf{0.06s} \\ 
        %  \hline 
        %  RePlan & 98.83 & 1.52 & 1.11 & 0.44s & 0.22s \\
        % \hline 
        %  NoFree & 87.83 & 1.43 & 1.06 & 0.74s & 0.42s \\ 
         \hline
    \end{tabular}
    \vspace{-0.15in}
    \label{tab:dset1}
\end{table}

\begin{figure}[ht]
    \begin{subfigure}{0.49\hsize}
       \centering    \includegraphics[width=0.9\textwidth, height = 2.6cm]{figures/vary-errors-1.png}
       % \caption{(a}
       % \label{fig:graphs1}
    \end{subfigure}
    \begin{subfigure}{0.49\hsize}
       \centering    \includegraphics[width=0.9\textwidth, height = 2.6cm]{figures/vary-errors-2.png}
       % \caption{(a}
       % \label{fig:graphs1}
    \end{subfigure}
    \caption{
        \footnotesize{
            {\textbf{Robustness to increasing number of errors}: Experiments analyse the recovery accuracy and time to generate a recovery plan with an increasing number of introduced errors }
        }
    }
    \label{fig:graphs}
    \vspace{-0.15in}
\end{figure}

%
\textbf{Plan Recovery with Compounding Errors. }
%
Table \ref{tab:dset2} reports the performance of various models on Data set 2, where a single randomized error occurs after each step in the original plan ($N_{err}=1$). Figure \ref{fig:graphs-2} shows the recovery accuracy against an increasing number of steps. Our model can recover a significantly larger part of the original plan, due to its high recovery accuracy and rapid re-planning ability. 
%

\begin{table}[ht]
    \centering
    \caption{Performance comparison when errors compound over time. }
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
         Model & Rec. \% & $L$ & $L/L_{opt}$ & 
         $T$ &
         $T/L_{opt}$ & Compl. \% \\ 
         \hline
         \hline
         Ours & \textbf{99.85} & 2.43 & 1.06 & \textbf{0.11s} & \textbf{0.04s} & \textbf{99.68} \\ 
         \hline 
         RePlan & 98.46 & 2.42 & 1.06 & 0.46s & 0.17s & 96.67 \\
        \hline 
         NoFree & 89.50 & 2.40 & 1.04 & 2.43s & 0.59s & 77.03 \\ 
        %  \hline
        %  Ours & \textbf{99.85} & 2.68 & 1.16 & \textbf{0.18s} & \textbf{0.06s} & \textbf{99.68} \\ 
        %  \hline 
        %  RePlan & 98.46 & 2.60 & 1.12 & 0.74s & 0.24s & 96.67 \\
        % \hline 
        %  NoFree & 89.50 & 2.41 & 1.05 & 2.40s & 0.58s & 77.03 \\ 
         \hline
    \end{tabular}
    \label{tab:dset2}
\end{table}


\textbf{Plan Recovery with Increasing Number of Objects. }
%
Table \ref{tab:dset4} reports the performance on Data set 3, where the scenes contain $6-10$ objects. We also study the variation of accuracy with an increasing number of objects in figure \ref{fig:graphs-2}. The proposed approach generalizes well to larger scenes owing primarily to discrepancy awareness and the use of learned heuristics (e.g., free space sampler) during plan search. 

\begin{table}[ht]
    \centering
    \caption{Performance comparison on larger scenes }
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
         Model & Recovery \% &  $L/N_{err}$ &  $L/L_{opt}$& $T/N_{err}$& $T/L_{opt}$  \\ 
         \hline
         \hline
         Ours & \textbf{93.77} & 4.60 & 1.06 & \textbf{0.94} & \textbf{0.19}\\ 
         \hline 
         RePlan & 92.09 & 4.59 & 1.03 & 1.63 & 0.29 \\
        \hline 
         NoFree & 65.35 & 4.50 & 1.02 & 7.02 & 1.12 \\ 
         \hline
        %  Ours & \textbf{93.77} & 5.09 & 1.21 & 4.62 & 0.80\\ 
        %  \hline 
        %  RePlan & 92.09 & 4.85 & 1.13 & 4.48 & 0.76 \\
        % \hline 
        %  NoFree & 65.35 & 4.52 & 1.02 & 6.87 & 1.10 \\ 
        %  \hline
    \end{tabular}
    \label{tab:dset4}
    \vspace{-0.1in}
\end{table}

\begin{figure}[ht]
    \begin{subfigure}{0.49\hsize}
       \centering    \includegraphics[width=0.9\textwidth,height = 2.6cm]{figures/vary-steps-1.png}
    \end{subfigure}
    \begin{subfigure}{0.49\hsize}
       \centering    \includegraphics[width=0.9\textwidth,height = 2.6cm]{figures/incobjects.png}
    \end{subfigure}
    \caption{
        \footnotesize{
            {\textbf{Plan Recovery Scalability.} Experiments analyse the reachability of the final goal in long-horizon plans and with an increasing number of objects. The graphs show that the proposed recovery method (in red) performs effectively for long-horizon plans and can scale to larger scenes as compared to the baselines.}
        }
    }
    \label{fig:graphs-2}
    \vspace{-0.2in}
\end{figure}

\begin{table}[h]
    \centering
    \caption{Recovery plan synthesis with any time search. 
    The use of heuristic-guided forward search to the nearest state in the anytime version results in an improvement in re-plan quality (shorter plans). The recovery plan quality improves with increasing the re-planning budget ($K$).} 
    \begin{tabular}{|c|c|c|c|}
    \hline
         Model & Recovery \% & $L_{plan} / L_{orig}$ & $T/N_{err}$\\ 
         \hline
         % \hline
         % Ours & & \textbf{1.00} & \\ 
         %\hline
         Anytime, K = 1 & 95.76 & 0.77 & 0.10s \\
        \hline 
         Anytime, K = 3 & 95.07 & 0.70 & 0.11s\\ 
         \hline
         Anytime, K = 5 & 94.52 & 0.64 & 0.15s\\ 
         \hline
    \end{tabular}
    \label{tab:dset3}
\end{table}

\textbf{Analysis Anytime Variant.} 
%
For evaluating the anytime version of our approach, we consider a subset of Data set 3 containing $6-8$ objects. Table \ref{tab:dset3} reports the performance of our original and anytime algorithms with increasing value of the planning budget, $K$ as ${1,3,5}$. 
%
Note: in these experiments reported, the heuristic distance from a candidate sub-goal on the original plan and the true goal are approximated as being equal.
%
The evaluation metric $L_{plan}/L_{orig}$ represents the ratio of the length of the recovery plan (for the given algorithm) to the length of the recovery plan in the case of the original algorithm. 
%
With increasing $K$, this ratio \emph{decreases}, indicating more efficient plans. However, the time to plan \emph{increases}, contributing to a smaller recovery accuracy illustrating the inherent length-time trade-off. 
%

\textbf{Error Detection Accuracy.}   
The total error detection accuracy is $94.5\%$ ($99\%$ recall and $79\%$ precision) on the evaluation data set. The accuracies of contributing modules are: (i) $88.2\%$ for object matching, (ii) $94.2\%$ for correctly detecting the pre-conditions and (iii) $98\%$ for correct outputs of the scene graph discriminator. 

\begin{figure}[ht]
    \begin{subfigure}{0.49\hsize}
       \centering    \includegraphics[width=0.9\textwidth, height = 2cm]{figures/rze_i.png}
       % \caption{(a}
       % \label{fig:graphs1}
    \end{subfigure}
    \begin{subfigure}{0.49\hsize}
       \centering    \includegraphics[width=0.9\textwidth, height = 2cm]{figures/rze_pre.png}
       % \caption{(a}
       % \label{fig:graphs1}
    \end{subfigure}
    \caption{
        \footnotesize{
            {\textbf{Predictions of \textit{free}-space module}. The figure on the left shows the initial scene where the task is to move the \textit{cyan lego} to a collision-free position. The figure on the right shows the predicted collision-free position for the \textit{cyan lego}. (yellow bounding box)}
        }
    }
    \label{fig:graphs}
    \vspace{-0.2in}
\end{figure}

\textbf{Qualitative results Results. }
Figure \ref{fig:qual-1} demonstrates our approach on a simulated 7-DOF Franka Emika robot manipulator in a simulated table-top setting. The execution of the original 4-step plan is erroneous due to the collision of the robot arm with the tower of blocks during the last step. The discrepancy between the actual and predicted scene graphs is detected and a 3-step recovery plan restores the blocks to their original positions.
%
Figure \ref{fig:qual-2} demonstrates the advantage of anytime recovery. After the first step of a 4-step plan, an external agent performs the next two steps. Instead of recovering to the current predicted state and unnecessary unstacking, the anytime recovery method identifies the state as being similar to the sub-goal after performing three steps, and thus, only the final step is performed.


==> sections/introduction.tex <==
\section{Introduction}\label{sec:intro}
%
An essential aspect of robot plan execution is \emph{recovering} from errors. While plans may be perfect in simulation, they are often marred by imperfections in the real world caused by sensor noise, motor failures, unexpected collisions or external disturbances. This results in deviations from the original path of planned execution, which the robot needs to recover from.
%
Consider a scenario where the robot is assigned the task of constructing a tower by stacking blocks on top of each other. Figure 1 illustrates a situation where the robot collides with a portion of the tower, causing the entire structure to collapse. It's important to note that recovering from such an error requires multiple actions to restack the blocks. 
%
In order to effectively recover from such complex errors, the robot should possess the ability to imagine the intended effects of its actions and compare them with the actual state reached to identify the \emph{sources} and \emph{degree} (or complexity) of the error. 
%
Once an error is detected, an efficient plan repair is necessary to return to a nominal state in the original plan, accommodating progress made before the error. Intuitively, the robot must optimise the \emph{replanning} effort to reach a nominal state in the intended plan that has progressed as far as possible towards the goal. 
%
% Often, efficiency becomes a vital consideration, both in terms of the time required to recover from error (in terms of the replanning) and the time it takes for the new plan to reach the goal state.

Error recovery in classical task planning~\cite{fox2006plan,bercher2014plan,saetti2022optimising} detect errors by explicit symbolic reasoning, such as checking the precondition of the next action in the plan, and recover through replanning to the original goal or last correct state.
% 
% The reliance on an accurate symbolic state causes brittleness due to uncertainty in action outcomes and perceptual noise. 
%
Alternate approaches for planning under uncertainty use reinforcement learning~\cite{thananjeyan2021recovery,vatsefficient,li2021reactive} to learn a reactive policy for the robot to recover from a deviant state to a nominal state. However, learning such a policy requires extensive offline exploration of error states, which is challenging in complex manipulation domains (verified in our experiments). 


Recently, \emph{learning-to-plan} methods have gained popularity because of their scalability to long horizons while being able to learn state and action representations from data. These methods learn to predict a plan - essentially a sequence of symbolic actions - to reach a goal specified through language instruction \cite{Kalithasan2022LearningNP, wang2023progport, zhu2021hierarchical, xu2019regression} or logical expression\cite{mao2022pdsketch}. Their training is usually supervised through a dataset comprising demonstrations of goal-reaching plans.   
%
A key limitation in these approaches is the absence of a feedback mechanism to assess goal attainment, resulting in the neglect of errors during execution. While some, like \cite{mao2022pdsketch}, use failure annotation data to learn to verify goal attainment, they fall short in monitoring individual action execution. Moreover, error recovery in such formalisms is largely cast as re-planning directly to the goal, disregarding prior planning efforts in producing the original plan.


In response, our work addresses the challenge of monitoring and recovering from errors during the execution of symbolic multi-step task plans generated by learning-to-plan methods. Additionally, we aim to learn to detect and recover from failures solely using demonstrations of goal-reaching plans, without any additional failure annotations.
%
Designing such an error recovery mechanism opens up two key questions: Firstly, \emph{``Can we learn a state discrimination function capable of identifying and localising differences between states in a self-supervised way without the need for manually annotated data?"} An affirmative answer to this question would presumably help in building an efficient and scalable error recovery mechanism. 
%
Further, \emph{``How can we leverage localised information about the failure to efficiently reach the original goal while minimising the replanning time and re-use a part of the original plan as appropriate"}. Our proposed work affirms both questions, presenting an efficient approach to recovering from plan failures.

% Introduction Figure. 
\begin{figure}[t!]
    \begin{subfigure}{1.0\hsize}
         \centering    
         \includegraphics[width =\textwidth, height = 4cm]{figures/Intro_new.png}
    \end{subfigure}
    \caption{
        \footnotesize{
            \textbf{Error Recovery.}  
             (Left) Errors in robot plan execution can be adversarial, cooperative or small perturbations arising from imperfect action execution. (Right) The recovery plan $\pi_{S_E}$ attains a state in the original intended plan $S_k \in tr(\Pi)$, preserving the progress already made with the shortest plan from the erroneous state $S_E$ to $S_k$ (equivalently within a planning budget). 
             %can be obtained by a replanning to the goal from scratch, which is expensive, or through a repair to the nearest state in the tr(Π)tr(\Pi), thus reusing the previous planning efforts. 
        }
    }
    \vspace{-0.2in}
    \label{fig:nsrm}
\end{figure}

%
We represent the world as a scene graph over neural object representations. 
%
Our key insight is to learn (i) a scene-graph transition model predicting the next scene graph for an input action; providing a foresight into how the scene will look as the plan is executed, and (ii) \emph{neural discriminators} to distinguish between two states as well as object representations. 
%
The discriminator trained in a \emph{self-supervised} way serves a dual role: it identifies the objects that are responsible for the failure and serves as a heuristic between states by discriminating object representations. 
%
The recovery plan is synthesised via a directed plan search towards a sub-goal, in the original plan, closest to the error state while being faithful to the progress achieved prior to the error. The search for the recovery plan is (i) \emph{neuro-symbolic} with explicit symbolic search operating over neural action models and (ii) \emph{discrepancy}-aware using context of erroneous object states during plan search.  

The approach is evaluated on a data set of simulated robot execution errors such as grasp failure during transport, adversarial/cooperative interventions in the scene and non-determinism in action outcomes due to motion planning errors. 
%
Experiments demonstrate rapid and accurate recovery from errors in multi-step plans (marred by sequential errors with multiple perturbations in a single step). The approach improves over (i) an RL-based approach which has been trained to reach the goal in a reactive manner and (ii) a full replanning approach adapted from ~\cite{mao2022pdsketch} in terms of the time taken to reach the sub-goal for recovery.
